Dyna-T: Dyna-Q and Upper Confidence Bounds Applied to Trees

In this work we present a preliminary investigation of a novel algorithm called Dyna-T. In reinforcement learning (RL) a planning agent has its own representation of the environment as a model. To discover an optimal policy to interact with the environment, the agent collects experience in a trial and error fashion. Experience can be used for learning a better model or improve directly the value function and policy. Typically separated, Dyna-Q is an hybrid approach which, at each iteration, exploits the real experience to update the model as well as the value function, while planning its action using simulated data from its model. However, the planning process is computationally expensive and strongly depends on the dimensionality of the state-action space. We propose to build a Upper Confidence Tree (UCT) on the simulated experience and search for the best action to be selected during the on-line learning process. We prove the effectiveness of our proposed method on a set of preliminary tests on three testbed environments from Open AI. In contrast to Dyna-Q, Dyna-T outperforms state-of-the-art RL agents in the stochastic environments by choosing a more robust action selection strategy.

==> input/experiments.tex <==
As mentioned earlier, StarCraft II used as the simulation environment. The simulations were done in MoveToBeacon map focusing on micro-management. For the evaluation of the performance of our algorithm we differed few parameters as to get results with regards to optimal performance and speed in both deterministic and stochastic environment.

\subsection{Deterministic environment}


\subsubsection{Maximizing reward}
The algorithms were tested for their ability to reach an optimal policy over 5000 episodes. All of them stabilized after the first thousand episodes and they kept that trend throughout the training without any changes. As seen in figure \ref{fig:5k} DynaQ+UCT reached picked at 25 average reward, followed by one step Q-Learning and DynaQ with 19 and 14 respectively. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/5k.png}
    \caption{In this graph we see the average reward for each algorithm for each of the 5000 episodes. The agent is allowed a maximum of 400 steps per episode, while for Dyna we have 10 planning steps per iteration.}
    \label{fig:5k}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/5ks.png}
    \caption{Standard deviation (std), computed in 500, 2000, 3500,
4500, and 5000 episodes. At 5000 episodes with the mean at 25, DynaQ+
UCT has a standard deviation of 14.8\% of the data. Q-learning
with mean at 18 got 38.8\% and DynaQ with average at 13 got 61.5\%.}
    \label{fig:5kstd}
\end{figure}


\subsubsection{Learning speed}
Speed test was created to evaluate the ability of our implementation into converging to a better policy faster. In figures \ref{fig:400},\ref{fig:400std} the algorithms were taking advantage of 400 steps per iteration while in \ref{fig:250} and \ref{fig:250std} we reduce that number to 250 steps per iteration. DynaQ+UCT led the way in every scenario we tried. It is worth to mention that reducing the steps allowed for one run resulted in reducing the average reward, thus the optimal agent's behavior. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/400e.png}
    \caption{Average reward for Q-Learning, Dyna-Q and DynaQ+
UCT for 500 episodes. A total of 400 steps are permitted for
the agent per each iteration.}
    \label{fig:400}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/400s.png}
    \caption{Standard deviation for 400 steps. While Q-learning is
stable with 22\% std and an average of 22, Dyna-Q has a massive std
of 61.5\% with mean 13. Combined with UCT, Dyna converges at 24
mean with only 20\% of std which forms the best performance.}
    \label{fig:400std}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/250e.png}
    \caption{Performance of the three algorithms with reduced maximum
steps per episode (250 steps). DynaQ+UCT and Q-Learning are
nearby by the end of 500 episodes, while DynaQ converged faster but
to a lower point.}
    \label{fig:250}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{input/250s.png}
    \caption{Standard deviation for 250 steps per iteration. As illustrated
from the data, DynaQ+UCT converged to a mean of 22 but with
38\% std, while one point lower, 21, Q-learning had less variation on
its data, 33\%. DynaQ, despite converging faster than the two others,
still had a wide variation of 57\% and 14 mean.}
    \label{fig:250std}
\end{figure}


\subsection{Stochastic environment}
\subsubsection{Maximizing reward}


\subsubsection{Learning speed}
